Ethical Considerations for Machine Translation of Indigenous Languages: Giving a Voice to the Speakers

In recent years machine translation has become very successful for high-resource language pairs. This has also sparked new interest in research on the automatic translation of low-resource languages, including Indigenous languages. However, the latter are deeply related to the ethnic and cultural groups that speak (or used to speak) them. The data collection, modeling and deploying machine translation systems thus result in new ethical questions that must be addressed. Motivated by this, we first survey the existing literature on ethical considerations for the documentation, translation, and general natural language processing for Indigenous languages. Afterward, we conduct and analyze an interview study to shed light on the positions of community leaders, teachers, and language activists regarding ethical concerns for the automatic translation of their languages. Our results show that the inclusion, at different degrees, of native speakers and community members is vital to performing better and more ethical research on Indigenous languages.

==> origsec3.tex <==
\section{On the Ethics of Research and How to Apply them to MT}
\label{sec:theory}

In recent times the discussion on ethics in NLP has gained interest, as the advances of the field are having a high impact on the life of millions of people around the globe. However, the ethics field is still in continuous debate. There are three big schools among ethicists: ``the actor’s moral character and dispositions (\textit{virtue ethics}), the duties and obligations of the actor given their role (\textit{decontology}), or the outcomes of the actions (\textit{consequentialism})'' \cite{Schnoebelen2017}. We will mention some basic statements from each school, so we can apply its visions during the paper. 

On the side of \textit{virtue ethics}, we can take Plato. For him, the ethical attitude of the person is based on the perception of the true nature of things, which is the presupposition of virtue, especially since true knowledge is to be sought in the higher and finds inner satisfaction therein \cite{Vorlander1903}. 

As the founder of the \textit{decontology}, we can take Kant. He states that the obligation arises from the unselfishly pursuing the good, whereby the goodwill should not be regarded as a means for the purpose but as the good that rests in itself. Therefore, moral action is what counts, not the outcome \cite{Kant1785}. They will hereby act as a practical reason, which can be guided by the categorical imperative: ``Act as if the Maxim should become the general law of nature through your will'' \cite{kant1870grundlegung}. This line of thought evolved into setting up a set of rules, codes of conduct, principles, or maxims that distinguish an action's morality. 

Finally, we have the \textit{consequentialists}, like Aristotle, that emphasizes the result of moral action. It refers to the pursuit of happiness (eudaimonia) that occurs after an action listed on the moral pursuit of values \cite{delosrios2014}, whereby virtue must be understood as a mean to an end \cite{muller2009gluck}. 

The practicality of having a set of rules or maxims is undeniable. However, it is possible that our vision might be constrained and oversimplified. Therefore, in this work, we aim to see the problem as diverse and complex. Norm based is not the only part in the equation of ethics and other factors need to be included representation, of communication, of service \newcite{chesterman2001proposal}. 


%\subsection{Ethics in the documentation and data collection process}
\subsection{Ethics and Data}
\label{subsec:ethics_documentation}

The study of endangered languages in indigenous communities has a long history in the last decades. The most prominent questions arise on the challenge of data collection \cite{smith2021decolonizing}. 

One of the common forms of this is to use normative ethics (decontology). Some relevant guidelines are the ones from The Australian Institute of Aboriginal and Torres Strait Islander Studies \footnote{\url{https://www.jstor.org/stable/pdf/26479543.pdf}}; the Ethical statement of the Linguistic Society of America \footnote{\url{https://www.linguisticsociety.org/content/lsa-revised-ethics-statement}-approved-july-2019}; and the DOBES code of conduct\footnote{\url{https://dobes.mpi.nl/ethical_legal_aspects/DOBES-coc-v2.pdf}}. These lists are a result of a broad and comprehensive discussion over decades in the field, where also indigenous voices inside academia raised \cite{smith2021decolonizing}. 

But why do we have so many attempts to set up an ethical code for the linguistic fieldwork? When it comes to working with human societies, there are no easy solutions for the ethical dilemmas that arise \cite{dwyer2006ethics}. Every situation requires special treatment and require compromise. This is why, in addition to the creation of an as general as a possible framework, the concrete application of such principles involves discussion. \newcite{dwyer2006ethics} suggests keeping track of the ethical issues and concerns during the documentation and the way these issues were solved, so other researchers can learn from this experience. A code of conduct or principles is good, but it might have the danger of an excess of regulations or even an inadequate regulation relegating this needed discussion. 

Overall, we can summarize the principles that appear in all suggested lists in three big themes:
\begin{itemize}
    \item \textit{Consultation, Negotiation and Mutual Understanding}. The right to consultation of indigenous people is stipulated in the convention 167 of the International Labor Organization \cite{ilo1989c169} and states that they ``have the right to right of indigenous peoples to preserve and develop their own institutions, languages, and cultures''. Therefore, informing the community about the research, negotiating a possible outcome, and reaching a mutual agreement on the directions and details of the research should be a default process.
    \item \textit{Respect to the local culture and involvement}. As each community has its own culture and view of the world, the researcher should be aware of it, as well as any intern governing organizations that might be interested in participating in the project or be informed. Also, it should be recommended that local researchers, speakers, or intern governments should be involved in the project.
    \item \textit{Share and distribute data and research}. The product of the research should be available for the usage of each community, so they can take advantage of the generated material like paper, books, or data. Also, non-technical versions of the research might help to give back the research.
    
\end{itemize}
Some of these commonly agreed principles are open to an agreement and might not be easy to solve in a general way. For instance, the documentation process will create data, and the ownership of this data is a major source of discussion. Here the traditional views of the communities might have a controversy with the juridical system of each country \cite{daes1993discrimination}. The problem is not easy and needs to be carefully considered when collecting data. 

A final aspect that is the call to de-colonization of research. The basic idea is that indigenous communities should be stopped from being seen as data sources and seen as people with their own history and will \cite{smith2021decolonizing}. The divorce between researchers and the cultural units of the communities can lead to reinforcing colonial legacy \cite{leonard2020producing}. 


\subsection{Ethics of translation}
\label{subsec:ethics_translation}

For a successful translation, the complete inclusion of all participants is important. Their equal participation, informal and understanding-oriented participation \cite{nissing2009grundpositionen}. Moral-practical discourses are based on proposals for norms by the communication community without any repression, which are in the same interest and express a general will. ``In this sense, the will of reason arguing determined by moral reasons does not remain external; the autonomous will is completely internalized to reason'' \cite{habermas1991erlauterungen}. 
So we can speak of ethical decisions if we incorporate others (developers of SMT systems, source text writers, translators, commissioners, post-editors, trainee translators, translation teachers, and consumers of machine translation) in the translation work \citep{kenny2011ethics}). For \newcite{rachels1986elements}, the minimum conception of morality is that when we give ``equal weight to the interests of each individual affected by one’s decision''. He approaches the question of how it should be presented authors’ intentions/text, the otherness of the source culture/author/text, the culturally-specific values, and norms in the best way \cite{chesterman2001proposal}. According to \newcite{doherty2016translations}, ``the translation process studies emerged to focus on the translator and the process of translation rather than on the end product'', incorporating mixed-method designs to get objective observations. For this they need a ``widespread recognition within the translation community'', like user-generated translation \cite{o2009evolution} online community translation \cite{o2011community} and open translation \cite{depalma2008translation}. So we can reach more quality, and ethical factors of this digital ontogenesis \cite{drugan2011translation}. 

A well-documented example of non-ethical translation usage is the one used as an instrument for colonial domination. The main aim was to ``civilize of the savages'' \cite{ludescher2001instituciones}. The Summer Institute of Linguistics (SIL International)\footnote{SIL International describes itself as ``.. a global, faith-based nonprofit that works with local communities around the world to develop language solutions that expand possibilities for a better life. SIL's core contribution areas are Bible translation, literacy, education, development, linguistic research, and language tools''. \url{https://www.sil.org/}} was used for this goal during the XX century in countries with indigenous cultures, translating the bible and trying to provoke a cultural change in these communities \cite{delvalls1978instituto,errington2001colonial,carey2010lancelot}. Of course, these practices are not new and have been practiced throughout history \cite{gilmour2007missionaries}. It is essential to notice that non-ethical research can still deliver useful material and knowledge, like language revitalization \cite{premsrirat2003language} but might inflict harm to the targeted community (\textit{consequentialism}). 

According to Habermas, the ethical and moral-practical discourse needs to be reconsidered when it comes to the exchange of different cultures and the translation of different languages. ``The reflexivity of modern world interpretations, therefore, does not establish, as Rawls and the liberal tradition assume, a superiority over the traditional understanding of the world.'' \cite{habermas1991erlauterungen}.

%%%%% Up to here

\subsection{The additionally challenges for machine translation}
\label{subsec:ethics_MT}

In the machine translation, we also must consider the ethical topics, like virtues and duties will be considered; however, in the NLP research, human subjects are not directly involved when the model is trained \citep{pavlick2014language}. Therefore, the process of data collection \cite{fort2011crowdsourcing}, evaluation \cite{couillault-etal-2014-evaluating} and the entire training process is vital.

Data collection is the first and most evident issue when it comes to translation. Modern NMT systems require a high amount of parallel data to be trained optimally \cite{junczys2019microsoft}. One way to obtain data is from crowd-sourcing \cite{fort2011crowdsourcing}. However, this kind of job is ill-paid and might constitute a problem for the living conditions of the workers \cite{schmidt2013good}.  
Also, data privacy is not trivial to handle. Systems must be able to avoid filtering sensitive information. 

The bias problem, like gender bias \cite{stanovsky2019evaluating} is also an ethical concern for MT.
It is also needed to disclose clearly the limitations and issues with certain systems \cite{leidner-plachouras-2017-ethical}. Being transparent is fundamental.

The NLP research can also be used as a political instrument of power, where we can observe mutual relationships between language, society, and the individual that ``are also the source for the societal impact factors of NLP'' \cite{horvath2017language}. In this way, NLP translation can be applied as an instrument to changing the culture of minorities as in traditional translation (\S\ref{subsec:ethics_translation}). So colonizers used translation as means of imperial control and expropriation \cite{cheyfitz1997poetics,niranjana10siting}. The asymmetry of power is the cause of domination, where subaltern cultures are flooded with ``foreign materials and foreign language impositions'' is a real danger for minority cultures \cite{tymoczko2006translation}.
\newcite{schwartz2022primum} discuss the need to decolonize our scientific approach in the whole NLP community, expressing the need of the researchers to the cognizance of the history and the cultural aspects of the communities that speak these languages. Additionally, he proposes that our research should have an obligation to provide some benefit with our studies to the communities, an obligation of accountability (and therefore be in direct contact with their governing organizations), and an obligation of non-maleficence.

Finally, we also have that many translation systems nowadays are multi-lingual. Thereby  also  multi-cultural challenges surge \cite{hershcovich2022challenges}. Translations must take into account different values and even understandings of the process and the product of NLP and, therefore, MT.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=.8\textwidth]{imgs/plots.pdf}
    \caption{Study performed on 22 participants that are members of indigenous communities from the Americas. }
    \label{fig:results}
\end{figure*}
